Graph Neural Network Guided Local Search for the Traveling Salesperson Problem

Solutions to the Traveling Salesperson Problem (TSP) have practical applications to processes in transportation, logistics, and automation, yet must be computed with minimal delay to satisfy the real-time nature of the underlying tasks. However, solving large TSP instances quickly without sacrificing solution quality remains challenging for current approximate algorithms. To close this gap, we present a hybrid data-driven approach for solving the TSP based on Graph Neural Networks (GNNs) and Guided Local Search (GLS). Our model predicts the regret of including each edge of the problem graph in the solution; GLS uses these predictions in conjunction with the original problem graph to find solutions. Our experiments demonstrate that this approach converges to optimal solutions at a faster rate than three recent learning based approaches for the TSP. Notably, we reduce the mean optimality gap on the 100-node problem set from 1.534% to 0.705%, a 2x improvement. When generalizing from 20-node instances to the 100-node problem set, we reduce the optimality gap from 18.845% to 2.622%, a 7x improvement.

==> results_gen.tex <==
\begin{tabular}{lllC{1.5cm}C{1.5cm}C{3.2cm}}
\toprule
\multirow{2}*{Model} & \multirow{2}*{Problem} & \multirow{2}*{Method} & \multicolumn{2}{C{3cm}}{Optimality gap (\%)} & \multirow{2}*{Optimal solutions (\%)} \\
& & & Median & IQR &\\
\midrule
\multirow{4}*{TSP20} & \multirow{4}*{TSP50} & Kool et al. &  2.5270 & 2.1080 &                 0.5005 \\
&&Joshi et al. + Sampling & 28.2036 & 5.7565 &                 0.0000 \\
     &&de O. da Costa et al. &  3.2976 & 2.7561 &                 0.5005 \\
                   &&\textbf{Ours} &  \textbf{0.0000} & \textbf{0.0618} &                \textbf{73.1732} \\
\midrule
\multirow{4}*{TSP20} & \multirow{4}*{TSP100} & Kool et al. & 26.5113 &  4.6053 &                 0.0000 \\
&&Joshi et al. + Sampling & 89.1632 &  7.4764 &                 0.0000 \\
     &&de O. da Costa et al. & 32.9608 & 12.1003 &                 0.0000 \\
                   &&\textbf{Ours} &  \textbf{2.5129} &  \textbf{2.1176} &                 \textbf{1.2012} \\
\midrule
\multirow{4}*{TSP50} & \multirow{4}*{TSP100} & Kool et al. &  4.0025 & 1.6081 &                 0.0000 \\
&&Joshi et al. + Sampling & 56.7009 & 6.6427 &                 0.0000 \\
     &&de O. da Costa et al. &  2.2806 & 1.8278 &                 0.0000 \\
                   &&\textbf{Ours} &  \textbf{1.1577} & \textbf{1.4869} &                 \textbf{7.6076} \\
\bottomrule
\end{tabular}

==> tsp100.tex <==
\begin{tabular}{llr}
\toprule
            Method &    mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. & 1.958±1.064 &                 0.3000 \\
      Joshi et al. & 1.559±4.071 &                51.6000 \\
O. da Costa et al. & 1.534±1.098 &                 1.4000 \\
              Ours & 0.705±0.807 &                20.5000 \\
          Concorde & 0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp100_perf.tex <==
\begin{tabular}{lll}
\toprule
            Method & Computation time (s) & Optimality gap (\%) \\
\midrule
       Kool et al. &          0.356±0.007 &        2.368±1.185 \\
      Joshi et al. &          6.127±0.081 &        1.880±4.097 \\
O. da Costa et al. &         30.656±0.734 &        0.773±0.717 \\
              Ours &         10.108±0.175 &        0.698±0.801 \\
     Arnold et al. &         10.128±0.194 &        1.757±1.240 \\
          Concorde &          0.573±0.771 &        0.000±0.000 \\
             LKH-3 &          0.118±0.022 &        0.011±0.058 \\
  Nearest Neighbor &          0.010±0.000 &       25.104±6.909 \\
Farthest Insertion &          0.444±0.010 &       12.456±2.944 \\
      Local Search &          0.727±0.165 &        4.169±2.047 \\
\bottomrule
\end{tabular}


==> tsp20.tex <==
\begin{tabular}{llr}
\toprule
            Method &     mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. &  0.069±0.255 &                84.6000 \\
      Joshi et al. & 1.000±12.492 &                97.4000 \\
O. da Costa et al. &  0.002±0.027 &                99.0000 \\
              Ours & -0.000±0.000 &               100.0000 \\
          Concorde &  0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp20_100.tex <==
\begin{tabular}{llr}
\toprule
            Method &     mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. & 18.845±2.447 &                 0.0000 \\
      Joshi et al. & 67.684±9.360 &                 0.0000 \\
O. da Costa et al. & 33.620±8.669 &                 0.0000 \\
              Ours &  2.622±1.544 &                 1.2000 \\
          Concorde &  0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp20_100_sens.tex <==
\begin{tabular}{llr}
\toprule
           Method &    mean\_std &  Optimal solutions (\%) \\
\midrule
Local search only & 4.169±2.046 &                 0.3000 \\
 Edge weight only & 2.183±1.383 &                 2.2000 \\
   Top 5 features & 2.228±1.421 &                 2.2000 \\
\bottomrule
\end{tabular}


==> tsp20_20_sens.tex <==
\begin{tabular}{llr}
\toprule
           Method &     mean\_std &  Optimal solutions (\%) \\
\midrule
Local search only &  1.824±3.252 &                54.7000 \\
 Edge weight only & -0.000±0.000 &               100.0000 \\
   Top 5 features &  0.000±0.003 &                99.9000 \\
\bottomrule
\end{tabular}


==> tsp20_50.tex <==
\begin{tabular}{llr}
\toprule
            Method &     mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. &  0.908±0.842 &                11.9000 \\
      Joshi et al. & 28.917±8.806 &                 0.0000 \\
O. da Costa et al. &  3.507±2.129 &                 0.2000 \\
              Ours &  0.161±0.396 &                73.2000 \\
          Concorde &  0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp20_50_sens.tex <==
\begin{tabular}{llr}
\toprule
           Method &    mean\_std &  Optimal solutions (\%) \\
\midrule
Local search only & 3.357±2.602 &                 6.4000 \\
 Edge weight only & 0.082±0.254 &                82.1000 \\
   Top 5 features & 0.080±0.295 &                83.2000 \\
\bottomrule
\end{tabular}


==> tsp20_perf.tex <==
\begin{tabular}{lll}
\toprule
            Method & Computation time (s) & Optimality gap (\%) \\
\midrule
       Kool et al. &          0.038±0.005 &        0.069±0.255 \\
      Joshi et al. &          1.344±0.106 &        2.031±2.928 \\
O. da Costa et al. &         21.120±0.352 &        0.001±0.025 \\
              Ours &         10.010±0.008 &       -0.000±0.000 \\
     Arnold et al. &         10.009±0.008 &       -0.000±0.000 \\
          Concorde &          0.119±0.083 &        0.000±0.000 \\
             LKH-3 &          0.020±0.019 &        0.000±0.000 \\
  Nearest Neighbor &          0.000±0.000 &      17.448±10.209 \\
Farthest Insertion &          0.005±0.000 &        2.242±2.536 \\
      Local Search &          0.007±0.003 &        1.824±3.254 \\
\bottomrule
\end{tabular}


==> tsp50.tex <==
\begin{tabular}{llr}
\toprule
            Method &     mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. &  0.494±0.655 &                29.5000 \\
      Joshi et al. & 1.206±18.066 &                86.3000 \\
O. da Costa et al. &  0.268±0.492 &                48.7000 \\
              Ours &  0.009±0.069 &                96.2000 \\
          Concorde &  0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp50_100.tex <==
\begin{tabular}{llr}
\toprule
            Method &      mean\_std &  Optimal solutions (\%) \\
\midrule
       Kool et al. &   2.032±0.860 &                 0.0000 \\
      Joshi et al. & 57.484±10.781 &                 0.0000 \\
O. da Costa et al. &   2.325±1.221 &                 0.2000 \\
              Ours &   1.378±1.122 &                 7.6000 \\
          Concorde &   0.000±0.000 &               100.0000 \\
\bottomrule
\end{tabular}


==> tsp50_perf.tex <==
\begin{tabular}{lll}
\toprule
            Method & Computation time (s) & Optimality gap (\%) \\
\midrule
       Kool et al. &          0.124±0.006 &        0.494±0.655 \\
      Joshi et al. &          3.080±0.182 &        0.884±1.700 \\
O. da Costa et al. &         24.338±0.523 &        0.136±0.314 \\
              Ours &         10.037±0.039 &        0.009±0.069 \\
     Arnold et al. &         10.035±0.039 &        0.040±0.180 \\
          Concorde &          0.258±0.197 &        0.000±0.000 \\
             LKH-3 &          0.069±0.030 &        0.000±0.012 \\
  Nearest Neighbor &          0.002±0.000 &       23.230±7.968 \\
Farthest Insertion &          0.065±0.001 &        7.263±3.072 \\
      Local Search &          0.101±0.031 &        3.357±2.603 \\
\bottomrule
\end{tabular}


==> tsplib_50.tex <==
\begin{tabular}{lllllllll}
\toprule
Method & \multicolumn{2}{l}{Kool et al.} & \multicolumn{2}{l}{Joshi et al.} & \multicolumn{2}{l}{O. da Costa et al.} & \multicolumn{2}{l}{Ours} \\
Metric &     Time (s) &       Gap (\%) &      Time (s) &        Gap (\%) &           Time (s) &       Gap (\%) &      Time (s) &      Gap (\%) \\
nice\_name &              &               &               &                &                    &               &               &              \\
\midrule
eil51     &  0.132±0.003 &   1.163±0.116 &   3.154±0.013 &    4.753±0.000 &       28.353±0.043 &   0.165±0.000 &  10.060±0.028 &  0.790±0.000 \\
berlin52  &  0.135±0.001 &   0.557±0.085 &   3.164±0.019 &    8.656±0.000 &       33.995±0.031 &   1.009±0.243 &  10.039±0.050 &  0.000±0.000 \\
st70      &  0.209±0.001 &   1.126±0.008 &   4.166±0.012 &   40.475±0.000 &       25.459±0.081 &   0.525±0.081 &  10.078±0.058 &  2.547±0.000 \\
eil76     &  0.235±0.000 &   2.002±0.218 &   4.538±0.023 &   30.433±0.000 &       28.184±0.024 &   0.972±0.210 &  10.048±0.041 &  1.573±0.000 \\
pr76      &  0.233±0.001 &   0.732±0.053 &   4.504±0.019 &   22.199±0.000 &       42.523±0.056 &   3.903±0.400 &  10.047±0.051 &  0.196±0.000 \\
rat99     &  0.360±0.000 &   3.355±0.342 &   5.842±0.019 &   39.993±0.000 &       34.519±0.194 &   1.525±0.007 &  10.095±0.046 &  4.491±0.000 \\
kroA100   &  0.362±0.001 &   2.137±0.430 &   5.965±0.030 &   48.458±0.000 &       42.530±0.044 &  23.479±0.000 &  10.098±0.067 &  3.002±0.000 \\
kroB100   &  0.364±0.001 &   5.264±0.253 &   5.917±0.028 &   70.913±0.000 &       35.361±0.028 &   2.264±0.906 &  10.274±0.179 &  1.785±0.000 \\
kroC100   &  0.363±0.001 &   3.503±0.392 &   5.898±0.014 &   56.617±0.000 &       36.882±0.049 &   2.558±0.117 &  10.025±0.045 &  3.828±0.000 \\
kroD100   &  0.363±0.001 &   3.558±0.237 &   5.906±0.025 &   37.606±0.000 &       27.570±0.052 &   0.330±0.392 &  10.191±0.056 &  2.644±0.000 \\
kroE100   &  0.363±0.001 &   2.186±0.409 &   5.945±0.031 &   52.152±0.000 &       37.125±0.034 &   8.397±0.900 &  10.040±0.039 &  2.084±0.000 \\
rd100     &  0.362±0.000 &   2.307±0.309 &   5.901±0.022 &   64.505±0.000 &       31.062±0.028 &   0.373±0.000 &  10.160±0.047 &  3.569±0.000 \\
eil101    &  0.370±0.000 &   3.942±0.217 &   5.958±0.024 &   34.865±0.000 &       25.541±0.023 &   0.372±0.143 &  10.097±0.052 &  4.101±0.000 \\
lin105    &  0.394±0.000 &   4.101±0.383 &   6.188±0.022 &   67.825±0.000 &       42.717±0.362 &   5.097±1.525 &  10.209±0.060 &  1.832±0.000 \\
pr107     &  0.404±0.001 &   4.278±0.360 &   6.299±0.040 &   42.359±0.000 &       31.074±0.026 &   1.807±0.311 &  10.106±0.053 &  0.255±0.000 \\
pr124     &  0.515±0.002 &   5.474±0.313 &   7.312±0.022 &   71.628±0.000 &       31.916±0.030 &   4.934±1.241 &  10.333±0.057 &  1.279±0.000 \\
bier127   &  0.540±0.001 &  12.868±0.695 &   7.477±0.027 &   48.187±0.000 &       42.078±0.026 &   5.149±0.480 &  10.342±0.158 &  1.374±0.000 \\
ch130     &  0.567±0.001 &   6.824±0.492 &   7.641±0.022 &   81.640±0.000 &       36.861±0.044 &   0.933±0.006 &  10.392±0.509 &  3.116±0.000 \\
pr136     &  0.603±0.003 &   9.978±0.596 &   7.946±0.114 &   64.411±0.000 &       31.293±0.024 &   0.387±0.125 &  10.693±0.221 &  4.211±0.000 \\
pr144     &  0.659±0.001 &  11.805±0.549 &   8.507±0.025 &  106.528±0.000 &       34.003±9.786 &   3.131±0.278 &  10.061±0.087 &  2.154±0.000 \\
ch150     &  0.715±0.001 &  11.203±1.127 &   8.826±0.025 &   85.568±0.000 &       37.852±0.035 &   1.630±0.509 &  11.005±0.090 &  3.210±0.000 \\
kroA150   &  0.718±0.000 &  10.372±0.997 &   8.832±0.024 &   93.977±0.000 &       31.447±0.029 &   1.355±0.270 &  10.917±0.106 &  4.098±0.000 \\
kroB150   &  0.715±0.001 &  10.469±0.721 &   8.849±0.023 &   81.043±0.000 &       31.216±0.031 &   1.683±0.000 &   9.962±0.371 &  5.271±0.000 \\
pr152     &  0.726±0.001 &  18.060±0.837 &   9.005±0.032 &   98.273±0.000 &       31.112±0.033 &   0.100±0.000 &  10.202±0.623 &  0.563±0.000 \\
u159      &  0.785±0.001 &  13.586±0.984 &   9.375±0.046 &   90.850±0.000 &       31.161±0.035 &   0.665±0.747 &  10.028±0.109 &  5.067±0.000 \\
rat195    &  1.139±0.001 &  16.704±0.597 &  11.626±0.044 &   73.418±0.000 &       36.877±0.045 &   1.353±1.335 &  11.026±0.048 &  6.466±0.000 \\
d198      &  1.194±0.138 &  51.214±3.947 &  11.800±0.115 &   63.116±0.000 &       31.145±0.054 &   0.276±0.106 &  11.018±0.067 &  8.498±0.000 \\
kroA200   &  1.177±0.003 &  22.477±0.834 &  12.073±0.042 &  129.871±0.000 &       36.269±0.048 &   3.910±0.000 &  11.036±0.062 &  8.007±0.000 \\
kroB200   &  1.176±0.001 &  20.070±1.402 &  12.019±0.053 &  101.349±0.000 &       34.368±0.024 &   9.503±0.709 &  11.605±0.051 &  4.662±0.000 \\
\bottomrule
\end{tabular}


==> tsplib_time.tex <==
\begin{tabular}{lllllllll}
\toprule
Method & \multicolumn{2}{l}{Kool et al.} & \multicolumn{2}{l}{Joshi et al.} & \multicolumn{2}{l}{O. da Costa et al.} & \multicolumn{2}{l}{Ours} \\
Metric &     Time (s) &         Gap (\%) &     Time (s) &       Gap (\%) &           Time (s) &       Gap (\%) &     Time (s) &      Gap (\%) \\
nice\_name &              &                 &              &               &                    &               &              &              \\
\midrule
eil51     &  9.958±0.007 &     0.994±0.025 &  3.026±0.012 &   8.339±0.000 &        9.993±0.006 &   0.111±0.237 &  9.992±0.009 &  0.000±0.000 \\
berlin52  &  9.939±0.005 &     1.597±0.463 &  3.068±0.022 &  33.225±0.000 &        9.992±0.005 &   0.563±0.561 &  9.988±0.013 &  0.142±0.000 \\
st70      &  9.900±0.005 &     1.549±0.113 &  4.037±0.009 &  24.785±0.000 &        9.994±0.003 &   0.040±0.085 &  9.981±0.011 &  0.764±0.000 \\
eil76     &  9.940±0.010 &     1.848±0.003 &  4.303±0.021 &  27.411±0.000 &        9.994±0.004 &   0.117±0.303 &  9.987±0.014 &  0.163±0.000 \\
pr76      &  9.972±0.007 &     0.529±0.144 &  4.378±0.023 &  27.793±0.000 &        9.990±0.007 &   1.529±1.392 &  9.996±0.003 &  0.039±0.000 \\
rat99     &  9.812±0.009 &     2.115±0.237 &  5.559±0.016 &  17.633±0.000 &        9.990±0.006 &   0.293±0.536 &  9.948±0.013 &  0.550±0.000 \\
kroA100   &  9.942±0.007 &     3.586±0.223 &  5.705±0.018 &  28.828±0.000 &        9.989±0.008 &  18.313±0.000 &  9.974±0.013 &  0.728±0.000 \\
kroB100   &  9.938±0.004 &     4.316±0.241 &  5.712±0.018 &  34.686±0.000 &        9.991±0.006 &   1.199±0.245 &  9.984±0.032 &  0.147±0.000 \\
kroC100   &  9.852±0.045 &     0.818±0.041 &  5.641±0.013 &  35.506±0.000 &        9.992±0.005 &   0.846±1.765 &  9.964±0.041 &  1.571±0.000 \\
kroD100   &  9.953±0.006 &     2.018±0.180 &  5.621±0.024 &  38.018±0.000 &        9.994±0.004 &   0.991±0.397 &  9.973±0.036 &  0.572±0.000 \\
kroE100   &  9.950±0.005 &     1.336±0.070 &  5.650±0.026 &  26.589±0.000 &        9.991±0.004 &   2.350±2.092 &  9.969±0.022 &  1.216±0.000 \\
rd100     &  9.945±0.006 &     2.909±0.262 &  5.737±0.033 &  50.432±0.000 &        9.993±0.005 &   0.046±0.142 &  9.989±0.011 &  0.459±0.000 \\
eil101    &  9.783±0.004 &     2.349±0.138 &  5.790±0.018 &  26.701±0.000 &        9.995±0.004 &   0.387±0.096 &  9.989±0.010 &  0.201±0.000 \\
lin105    &  9.884±0.180 &     1.404±0.094 &  5.938±0.040 &  34.902±0.000 &        9.987±0.005 &   2.521±1.990 &  9.974±0.012 &  0.606±0.000 \\
pr107     &  9.874±0.004 &     2.632±0.547 &  5.964±0.048 &  80.564±0.000 &        9.993±0.003 &   0.926±0.391 &  9.961±0.023 &  0.439±0.000 \\
pr124     &  9.887±0.161 &     2.910±0.125 &  7.059±0.031 &  70.146±0.000 &        9.992±0.005 &  11.299±5.297 &  9.985±0.020 &  0.755±0.000 \\
bier127   &  9.737±0.272 &     5.306±0.377 &  7.242±0.022 &  45.561±0.000 &        9.994±0.007 &   3.233±0.737 &  9.981±0.015 &  1.948±0.000 \\
ch130     &  9.462±0.006 &     2.966±0.126 &  7.351±0.074 &  39.090±0.000 &        9.991±0.005 &   1.011±1.366 &  9.965±0.030 &  3.519±0.000 \\
pr136     &  9.456±0.004 &     3.939±0.448 &  7.727±0.026 &  58.673±0.000 &        9.990±0.005 &   0.443±1.401 &  9.980±0.008 &  3.387±0.000 \\
pr144     &  9.680±0.005 &     6.643±0.295 &  8.132±0.017 &  55.837±0.000 &        9.994±0.004 &   1.611±0.369 &  9.985±0.011 &  3.581±0.000 \\
ch150     &  9.840±0.004 &     3.921±0.341 &  8.546±0.048 &  49.743±0.000 &        9.990±0.005 &   0.366±0.181 &  9.979±0.010 &  2.113±0.000 \\
kroA150   &  9.818±0.004 &     3.400±0.140 &  8.450±0.017 &  45.411±0.000 &        9.990±0.004 &   0.829±0.365 &  9.936±0.057 &  2.998±0.041 \\
kroB150   &  9.843±0.004 &     2.008±0.166 &  8.573±0.021 &  56.745±0.000 &        9.995±0.003 &   0.973±0.503 &  9.948±0.031 &  3.297±0.082 \\
pr152     &  9.307±0.005 &     6.451±0.313 &  8.632±0.035 &  33.925±0.000 &        9.991±0.003 &   0.034±0.031 &  9.957±0.025 &  3.119±0.000 \\
u159      &  9.406±0.283 &     5.852±0.396 &  9.012±0.019 &  38.338±0.000 &        9.993±0.004 &   0.054±0.000 &  9.974±0.016 &  1.020±0.000 \\
rat195    &  8.983±0.002 &     6.531±0.222 &  0.000±0.000 &       nan±nan &        9.993±0.005 &   1.081±1.098 &  9.625±0.055 &  1.690±0.000 \\
d198      &  9.202±0.123 &  314.055±22.968 &  0.000±0.000 &       nan±nan &        9.992±0.004 &   1.140±1.970 &  9.917±0.026 &  6.513±0.020 \\
kroA200   &  9.281±0.005 &     6.446±0.244 &  0.000±0.000 &       nan±nan &        9.995±0.004 &   1.472±0.136 &  9.904±0.052 &  2.081±0.000 \\
kroB200   &  9.278±0.024 &     7.973±0.267 &  0.000±0.000 &       nan±nan &        9.993±0.004 &   2.338±1.117 &  9.959±0.039 &  2.589±0.000 \\
\bottomrule
\end{tabular}

